Joint Learning of 3D Shape Retrieval and Deformation

We propose a novel technique for producing high-quality 3D models that match a given target object image or scan. Our method is based on retrieving an existing shape from a database of 3D models and then deforming its parts to match the target shape. Unlike previous approaches that independently focus on either shape retrieval or deformation, we propose a joint learning procedure that simultaneously trains the neural deformation module along with the embedding space used by the retrieval module. This enables our network to learn a deformation-aware embedding space, so that retrieved models are more amenable to match the target after an appropriate deformation. In fact, we use the embedding space to guide the shape pairs used to train the deformation module, so that it invests its capacity in learning deformations between meaningful shape pairs. Furthermore, our novel part-aware deformation module can work with inconsistent and diverse part-structures on the source shapes. We demonstrate the benefits of our joint training not only on our novel framework, but also on other state-of-the-art neural deformation modules proposed in recent years. Lastly, we also show that our jointly-trained method outperforms various non-joint baselines.

==> sections/4approach.tex <==
\section{Method Details}
\vspace{-3pt}

We first describe our deformation module in \ref{deform_module}, then the embedding module in \ref{embedding_module}, and finally our joint training scheme in \ref{training_scheme}. 

\subsection{Joint Training Scheme}
\label{training_scheme}
We alternately update the embedding module and the deformation module during the joint training process. The aim is to leverage on the embedding module to select better source candidates $\{\mathbf{s}'\}$ for each target $\mathbf{t}$ in order to ``specialize" the deformation module. Let $M=|\{\mathbf{s}'\}|$. We use a biased selection of the $M$ source candidates for each target based on the current embedding distance values. The probability of sampling a particular source model for a given target is proportional to its current embedding distance, relative to other sources in the database. We show in our experiments that this biased sampling achieves better performance than random sampling. 

\leo{Don't we also need a subsection on what we do at test time? In particular, on how we select the best database CAD model (or models) to deform for the given query target?}
\mk{Given a target image/point cloud, we use the embedding space to retrieve the closest source model from the source model database at test time.}

\subsection{Deformation Module}
\label{deform_module}
In this subsection, the deformation function $\mathcal{D}$ assumes that a source shape $\mathbf{s}$ has been selected from the database of sources $\mathbf{B}$.

\subsubsection{Parametric Models}
Since most human designed objects can be easily decomposed into parts, a lot of shape variants can be made by leveraging on these. Hence deformations of our database source shapes $\mathbf{s_i}\in\mathbf{B}$ are parameterized by \emph{per-part axis aligned bounding boxes}. Each part has 6 parameters (3 for the box center and 3 for the scale). Examples are shown in Fig~\ref{fig:param_model}. We need to handle sources with different parameterizations, \ie different number of parameters, so for source shape $\mathbf{s_i}$ with $K_i$ parts, the output of the deformation module $\mathcal{D}$ are the decoded $(6 \times K_i)$ parameters for source $\mathbf{s_i}$ to fit the target that minimizes $l_{fitting}$.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{deformation_network.pdf}
    % \vspace{-0.5cm}
    \caption{Our deformation module network architecture.
    }
    \label{fig:network}
    \vspace{-1.5\baselineskip}
\end{figure}

\subsubsection{Network Architecture}
Our deformation network has to be able to handle models with varied number of parts. Our architecture is shown in Fig~\ref{fig:network}. The predicted per-part is conditioned on learned target latent codes $\mathbf{t}_{\mathcal{D}}$, source latent codes $\mathbf{s}_{\mathcal{D}}$, and per source part latent codes $\mathbf{s}_{\mathcal{D}}^{p_j}$. The predicted per-part parameters are then concatenated together to result in the final deformation parameters that outputs the deformed source shape. Conditioning on source per-part latent codes allows us to handle models with different number of output parameters as it predicts the deformation parameters for each part separately.

We use a PointNet encoder to encode the target shape and obtain the target latent code, \ie $\mathbf{t}_{\mathcal{D}} = \mathcal{E}_{\mathcal{D}}(\mathbf{t}) \in \mathbb{R}^{n_1}$. The source latent codes $\mathbf{s}_{\mathcal{D}} \in \mathbb{R}^{n_2}$, and per source part latent codes $\mathbf{s}_{\mathcal{D}}^{p_j} \in \mathbb{R}^{n_3}$, are directly optimized (\mk{autodecoded? not sure the right term)}, which we can do because we have a fixed database of shapes. Thus, the output deformation parameters $p_{s}^t$ for a target shape $\mathbf{t}$ and source shape $\mathbf{s}$ can be written as 
%
\vspace{-3pt}
\begin{equation}
    p_{s_j}^t = \mathcal{P}(\mathbf{t}_{\mathcal{D}}, \mathbf{s}_{\mathcal{D}}, \mathbf{s}_{\mathcal{D}}^{p_j}),
\end{equation}
%
and 

\begin{equation}
    p_{s}^t = [p_{s_1}^t, p_{s_2}^t, ..., p_{s_K}^t],
\end{equation}

\noindent where $\mathcal{P}$ is a lightweight series of MLP's.

\noindent \mk{Mention that we are predicting the offset from the default source parameter. Not yet included here.}\\

\noindent \textbf{Additional constrains and supervision}
Our choice of parametric model and deformation module design also allows us to leverage additional constraints and supervision. We pre-compute connectivity constraints for the source parametric models, this simulates information-rich databases that are expensive to construct, which supports our motivation to be able to create variations from these. The output of the deformation network is then projected using the connectivity constraint matrix that results in deformed models that maintain connectivity. Results show that this improves the performance of our approach.\\  

\noindent \textbf{Source models connectivity constraint}
The connectivity constraint is represented as a matrix that projects the output parameters onto the space that satisfies the pre-calculated connectivity of the source model, which is done by a simple matrix multiplication. Connectivity is pre-computed by first identifying part pairs that are connected, \ie distance between the closest pair of points (joint) is within a threshold. We then define the joint to be the midpoint of the closest pair of points, and obtain a linear constraint that enforces the joint to maintain its connection. We obtain a number of linear constraints from the collection of joints that results in a constraint matrix $B$. Let $N$ be the nullspace, \ie columns representing the null space basis vectors, of $B$, then the constraint projection matrix is given by $NN^T$.

\subsection{Retrieval Embedding Module}
\label{embedding_module}
The importance of the retrieval module is to be able to select a deformable source shape for a given target. We aim to achieve this by learning an embedding space $\mathcal{R}$. We use the same embedding representation as \cite{uy-deformawareretrieval-eccv20} and train an embedding to reflect the fitting error of the deformation module. We use a PointNet encoder to encode the targets into the embedding space $\mathbf{t}_\mathcal{R} \in \mathbb{R}^{n_4}$. We directly optimize for the retrieval source latent codes $\mathbf{s}_\mathcal{R} \in \mathbb{R}^{n_4}$ and source variance $\mathbf{s}_\mathcal{R} ^ v \in \mathbb{R}^{(n_4\times n_4)}$, which is represented by a diagonal positive definite matrix. A sigmoid activation function was used to ensure it is positive. Then as in \cite{uy-deformawareretrieval-eccv20}, the distance in the embedding space is given by

\begin{equation}
    d(\mathbf{s}, \mathbf{t}) = \sqrt{(\mathbf{s}_{\mathcal{R}}-\mathbf{t}_{\mathcal{R}})^{T}\mathbf{s}_{\mathcal{R}}^v(\mathbf{s}_{\mathcal{R}}-\mathbf{t}_{\mathcal{R}})}.
\end{equation}

The goal is to enforce the distance in embedding space $d$ reflects $l_{fitting}$ at some optimal state of the deformation module $\mathcal{D}$. For a target $\mathbf{t}$, if we have a set of selected sources $\{\mathbf{s}'\}$ and let $f$ be a function that reflects the \emph{similarity} between the values of $d$ and $l_{fitting}$, then we have 

\begin{equation}
    l_{embedding}(\mathbf{t}, \{\mathbf{s}'\}) = \sum_{\mathbf{s'}} (f(\ d(\mathbf{s'},\mathbf{t}),\ l_{fitting}(\mathcal{D}(\mathbf{s}',\mathbf{t}), \mathbf{t}))). 
\end{equation}

\noindent We use a regression based loss as $f$ similar to the regression based approach in \cite{uy-deformawareretrieval-eccv20}.

\mk{Should we right about: since the database is fixed and we are directly optimizing for the source latent codes then the network does not see the ``default" state of the parametric models. Does this have an advantage?}





==> sections/old/1introduction.tex <==
\section{Introduction}

\noindent \mk{Motivation for 3D content creation}

Creating and designing new 3D models is a tedious and difficult process even for expert designers. Hence automating 3D content creation is an important task. We want to create more high quality 3D models by leveraging on data available in the wild such as sparse point clouds, incomplete 3D scans and images. 

\noindent \mk{Use database + deformation}

However, direct generation or completion of shapes from scans or images result in artifacts and do not output in clean CAD models with sharp features as designed by artists. In order to achieve high quality models, we leverage on existing CAD repositories and 3D deformation techniques to learn shape variations from acquired data that may be sparse and incomplete. 

\noindent \mk{Not all shapes deformable to each other. Retrieval is important}

Due to the wide variations of shapes, such has differences in structure, topology and appearance, and regularizations and constraints of deformation techniques in order to preserve the integrity of the models, not all shapes are deformable to each other. At the very least, randomly selecting a source shape to deform to a given target might not be ideal for fitting. Thus, retrieving a deformable source given a desired target is important in creating high quality shapes for fitting.

\noindent \mk{Our proposed approach.} \mkbad{Why joint? This currently doesn't answer the importance of joint learning.}

In order to select the appropriate deformable shape given a target, the variations that can be achieved from each source shape, which is also information that we do not have and is not trivial to manually define. A previous work \cite{uy-deformawareretrieval-eccv20} use a fixed ARAP optimization objective as a deformation function, but this limits the variations to very local deformations. The range of variations is also fixed for each shape as specified by the objective function. We aim to learn more holistic and robust shape variations by leveraging on data and deep networks.Hence we propose a framework that jointly learns the embedding space for deformable shape retrieval and the shape deformation network. 

\noindent \mk{Why is it hard?}

This task is purely unsupervised because for each target shape, we do not know the ``ground truth" or optimal source model for it as we do not have the range of the variations of source shapes a priori. Moreover, given a particular source-target pair, we also do not know the optimal deformation parameters as the resulting deformed shape will not be a perfect fit due to constraints and regularizations. Thus, finding deformable sources is not an easy task and all previous deformation networks \cite{Yifan:NeuralCage:2020, wang20193dn} only train and test on random source-target pairs which is not ideal. 

\noindent \mk{Contributions}

Hence, it becomes a chicken-and-egg problem where if we have a bad fitting error, it can either be caused by a bad source selection or by a sub-optimal deformation function. \mkbad{Bad reason...} We propose a joint learning pipeline in order to strike a balance between the two objectives, that is, we want to models that fit to the target, preserve fine features and structures and learn larger variations from the sources. Thus our contributions are 

\begin{itemize}
    \item an unsupervised joint pipeline for both learning of a deformable shape retrieval space and a shape deformation network;
    \item a deformation module that is based on parametric models (axis-aligned part bounding boxes) that allows for the preservation of sharp features and is also able to handle different number of parameters; \mkbad{problematic.}
    \item we also demonstrate the usability of our proposed approach on various applications that allows for high quality 3D content creation.
\end{itemize}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/param_models.pdf}
    % \vspace{-0.5cm}
    \caption{Examples of our parametric model handles.
    }
    \label{fig:param_model}
    % \vspace{-1.5\baselineskip}
\end{figure*}

\mkbad{I think the two competing objectives should be 1) have bigger variations, which means deforming bad/far source-target pairs allows more variations. 2) Selecting good pairs so that we can maximize the capacity of the deformation network. But (naive) easy pairs won't give big variations.}


==> sections/old/5experiments.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/results.pdf}
    % \vspace{-0.5cm}
    \caption{(From left to right) Results for Tab~\ref{table:comparisons} and Tab~\ref{table:ablation}.
    }
    \label{fig:quantitative}
    % \vspace{-1.5\baselineskip}
\end{figure*}

\begin{table*}
    \centering
        \begin{tabular}{c|c|c|c|c|c}
        Method & Top 1 & Top 2 & Top 3 & Top 4 & Top 5\\
        \hline
        PC-ICP &  &  &  &  & \\
        PC-DF & 0.01053 & 0.01141 & 0.01205 & 0.01201 & 0.01239 \\
        PC-NC &  &  &  &  & \\
        RD-ICP &  &  &  &  & \\
        RD-DF & 0.01049 & 0.01091 & 0.01139 &  0.01191 & 0.01200\\
        RD-NC &  &  &  &  &\\
        \textbf{Ours} & \textbf{0.00987} & \textbf{0.01065} & \textbf{0.01112} & \textbf{0.01159} & \textbf{0.01182}\\ 
        \textbf{Ours-ICPL2} & \textbf{0.00944} & \textbf{0.01031} & \textbf{0.01105} & \textbf{0.01131} & \textbf{0.01150}\\
    \end{tabular}
    \caption{Mean Chamfer distance errors for top 5 \textbf{retrieval} on the chair class with source database of 500 chairs.
    \label{table:comparisons}}
\end{table*}

\section{Experiments}

\subsection{Implementation Details}
We used the StructureNet dataset on X object classes. \mk{Current results reported below are on the chair class.} We use 500 randomly selected source models as our parametric model database. We have 4824 and 1207 training and test targets, respectively. We pre-train our deformation module on random source-target pairs to initialize our joint training approach. If not specified, current results shown for our deformation module is uses the pre-computed connectivity constraint, and a simple chamfer distance is chosen as $l_{fitting}$, but we also ablate on with additional part-based loss supervision.

We alternate update our deformation module and our embedding module in our joint training scheme, and we select $M=10$ candidate sources for each target at each iteration. We start using our embedding distance based sampling after training the embedding module for 30 epochs on random samples.

\subsection{Results}
\subsubsection{Evaluation Metric}
There are two evaluation schemes of interest in the joint learning scheme: 1) mean fitting error of the deformed retrieved models to the target, which showcases how well the retrieval module and deformation module perform together; and 2) mean fitting error given an oracle retrieval module, which is the best fitting error achieved assuming perfect selection. This showcases how well the deformation network learns to fit \mk{and also shows how much variations the network learned that the sources can deform to}.\\

\noindent \mkbad{Plan: Still to build and run this experiment.}\\
\noindent \textbf{Evaluation for goodness of the retrieval module.} Use generated variations of the source models in the database as the test set in order to have ground truth ``cluster assignments" to evaluate retrieval performance. We can also evaluate the performance of the deformation module in capturing variations by calculating the mean fitting error on the correct retrievals.

\begin{table*}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
        Method & Top 1 & Top 2 & Top 3 & Top 4 & Top 5\\
        \hline
        PC-DF & 0.01053 & 0.01141 & 0.01205 & 0.01201 & 0.01239 \\
        PC-U-DF & 0.01139 & 0.01195 & 0.01214 & 0.01257 & 0.01328\\
        RD-DF  & 0.01049 & 0.01091 & 0.01139 &  0.01191 & 0.01200\\
        RD-U-DF & 0.01134 & 0.01238 & 0.01230 & 0.01319 & 0.01360\\
        RD-U-DF-ICPL2 &  &  &  &  &\\
        \textbf{Ours} & \textbf{0.00987} & \textbf{0.01065} & \textbf{0.01112} & \textbf{0.01159} & \textbf{0.01182}\\
        \textbf{Ours-ICPL2} & \textbf{0.00944} & \textbf{0.01031} & \textbf{0.01105} & \textbf{0.01131} & \textbf{0.01150}\\
    \end{tabular}
    \caption{Mean Chamfer distance errors for top K retrieval on the chair class with source database of 500 chairs. \label{table:ablation}}
\end{table*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/qualitative_results.pdf}
    % \vspace{-0.5cm}
    \caption{Examples of qualitative results of our joint retrieval and deformation approach. The triplets are in the order (source, target, deformed).
    }
    \label{fig:qualitative}
    % \vspace{-1.5\baselineskip}
\end{figure*}

\subsubsection{Baselines and Comparisons}
We compare our joint approach with baselines without a joint embedding and deformation approach that mimic the approaches from \cite{uy-deformawareretrieval-eccv20}. The first set of baselines use the same candidate selection procedure as in \cite{uy-deformawareretrieval-eccv20}, pre-compute the fitting gaps and then train an embedding space that reflect these fitting gaps.
\begin{itemize}
    \item The first baseline (\textbf{PC-ICP}) use the same parametric models and deformation handles as ours, but uses a direct optimization method, \ie no neural network, to achieve the final fitting parameters. The drawback of this approach is this pre-computation is computationally very expensive to do for multiple source-target pairs.
    \item The second baseline (\textbf{PC-DF}) uses the same deformation network as ours but keeps this network fixed and does not update it during the training of the embedding space. The deformation network was pre-trained on random source-target pairs prior to the training of the embedding space. The candidates used for training the embedding network are obtained using the similar method as in \cite{uy-deformawareretrieval-eccv20}.
    \item The third baseline (\textbf{PC-NC}) is the same as the second but replaces the parametric deformation network with Neural Cages \cite{Yifan:NeuralCage:2020}.
\end{itemize}

The second set of baselines randomly samples candidates on the fly instead of pre-selecting candidates as in \cite{uy-deformawareretrieval-eccv20}. We use both our parametric model based deformation network (\textbf{RD-DF}) and Neural Cages \cite{Yifan:NeuralCage:2020} (\textbf{RD-NC}). We also ran on the fly sampling with direct fitting (\textbf{RD-ICP}) for Y days, but the it is computationally very expensive \mk{should we compare with this?}. Results are shown in Tab~\ref{table:comparisons} and Fig~\ref{fig:quantitative}-left.

\subsubsection{Ablation Studies}
We run ablation studies on the different design choices of our approach. We update the deformation network instead of keeping it fixed, we ablate on both pre-computed candidates (\textbf{PC-U-DF}) and randomly sampled candidates (\textbf{RD-U-DF}). For our approach, we jointly update the embedding and deformation modules and we sample source candidates based on the current embedding distances instead of a random selection. This enables better selection of ``deformable" pairs for the deformation module learning. Additionally, we add an additional supervision for the deformation module of initializing with the network prediction and running an ICP post-fitting and updating the deformation with an L2 loss (\textbf{-ICPL2}). We also ablate this with the random sampling of sources. Results are shown in Tab~\ref{table:ablation} and and Fig~\ref{fig:quantitative}-right.

\begin{table*}
    \centering
        \begin{tabular}{c|c|c|c|c|c}
        Method & Top 1 & Top 2 & Top 3 & Top 4 & Top 5\\
        \hline
        Fixed & 0.00720 & 0.00820 & 0.00887 & 0.00932 & 0.00971\\
        PC-U-DF & 0.00711 & 0.00811 & 0.00876 & 0.00923 & 0.00961\\
        RD-U-DF & 0.00717 & 0.00814 & 0.00881 & 0.00927 & 0.00965\\
        RD-U-DF-ICPL2 &  &  &  &  &\\
        \textbf{Ours} & 0.00715 & 0.00804 & 0.00867 & 0.00914 & 0.00953\\
        \textbf{Ours-ICPL2} &  \textbf{0.00644} & \textbf{0.00733} & \textbf{0.00792} & \textbf{0.00833} & \textbf{0.00870}\\
    \end{tabular}
    \caption{Mean Chamfer distance errors for the \textbf{oracle} top 5 CD errors on the chair class with source database of 500 chairs.
    \label{table:oracle}}
\end{table*}

\subsubsection{Quantitative Results}
We shown some qualitative examples of our joint retrieval and deformation approach in Fig~\ref{fig:qualitative}. This shows that our approach is able to output clean CAD models given a target.

\subsubsection{Deformation Module Ablations}
Due to our choice of deformation module, we are able to leverage on additional supervision from the source models. We ablate on using the pre-computed connectivity constraints and projecting the output parameters of the deformation module onto the constraint space (\textbf{-conn}). Additionally, we also ablate on using a part-based chamfer loss that enforces the semantic labels to agree (\textbf{-pl}). Lastly, we also ablate on using the direct fitting post-processing (\textbf{-ICPL2}) that was initialized with the network prediction and supervised with an L2 loss. Results are shown in Tab~\ref{table:deformation_module}.

\begin{table}
    \centering
    \begin{tabular}{c|c|c|c|c}
        Method & Rnd & Top 1 & Top 2 & Top 3 \\
        \hline
        vanilla & 0.03236 & 0.00766 & 0.00880 & 0.00945 \\
        -conn & 0.02913 & 0.00719 & 0.00819 & 0.00887 \\
        -conn -pl & 0.02851 & 0.00660 & 0.00739  & 0.00803 \\
        -conn -ICPL2 & 0.02915 &  0.00720 & 0.00821 & 0.00888 \\

    \end{tabular}
    \caption{Mean Chamfer distance errors for an oracle ranking and for a randomly selected source, \ie no retrieval, for the deformation network. Note that this network has no embedding. \label{table:deformation_module}}
\end{table}

% \subsubsection{Joint Training Deformation Module Update Ablations}
% \mk{Is this section helpful? Leave out?}
% We also tried s

\subsection{Applications}
\mkbad{TODO}
\subsubsection{Scan2CAD}

\subsubsection{Image2CAD}

\subsubsection{Interpolation}
We can build a decoder in the retrieval embedding space that decodes the target geometry. This will enable us to interpolate through the embedding space to see the variations in the deformed geometry. The shape outputed by the decoder will be used as input target to the deformation module.

% \subsubsection{OLD}
% Here, for the deformation network we assume that we pre-train it on random source-target pairs and initialize the joint training module with this.

% \noindent \textbf{Flags to consider for the deformation module.}
% \begin{itemize}
%     \item with/without connectivity,
%     \item with/without part-loss,
%     \item with/with post-process direct supervision (ICP fitting) via L2 supervision.
% \end{itemize}

% \noindent \textbf{Comparisons for design of the joint training pipeline.}
% \begin{itemize}
%     \item Fixed vs not fixed deformation network as embedding network is trained.
%     \item {
%     Sampling of $M$ candidates per target in each iteration done by 
%     \begin{enumerate}
%         \item randomly,
%         \item embedding space distance probabilities.
%     \end{enumerate}
%     }
%     \item {
%     Update of (not fixed) deformation function based on
%     \begin{enumerate}
%         \item all sampled $M$ pairs (weighted by probabilities or simple mean in the random case),
%         \item only the minimum of $M$ samples,
%         \item within a threshold fitting error from the minimum of the $M$ samples.
%     \end{enumerate}
%     }
% \end{itemize}

% \noindent \textbf{Comparisons with variants of the ECCV work \cite{uy-deformawareretrieval-eccv20}}
% \begin{enumerate}
%     \item Given a fixed deformation network the same as in our joint pipeline, sample a fixed set of candidates for each target in the training set to train the retrieval embedding module. This uses the same sampling as in \cite{uy-deformawareretrieval-eccv20}, but simply changing the deformation module.
%     \item Change the deformation module to a direct fitting optimization (ICP), mimicing the ARAP deformation function as in \cite{uy-deformawareretrieval-eccv20}, but with the same parametric model setup.
%     \item Take another existing deformation network such as Neural Cages \cite{Yifan:NeuralCage:2020} to replace our bounding-box based deformation module. Check if joint training also improves the result when changing the deformation network.
% \end{enumerate}

% \noindent \textbf{Comparisons for retrieval performance.}
% To show that if there is an imporvement solely on the retrieval when joint training is done. Same baselines as in the ECCV work \cite{uy-deformawareretrieval-eccv20}.
% \begin{itemize}
%     \item Ranked CD,
%     \item AE,
%     \item region embedding.
% \end{itemize}

% \subsubsection{Parametric model database setups}
% Factors we need to consider for parametric model database
% \begin{itemize}
%     \item propagate to different object classes
%     \item vary the database size
% \end{itemize}

==> tables/tbl_diff_params.tex <==
\begin{table}
{
\footnotesize
\centering
\setlength\tabcolsep{2pt}
\begin{tabularx}{\linewidth}{c|CC|CC|CC}
    \toprule
    &\multicolumn{2}{c|}{Chair}&\multicolumn{2}{c|}{Table}&\multicolumn{2}{c}{Cabinet}\\
    \cline{2-7}
    & \scriptsize{Rank 1} & \scriptsize{Rank 3}  & \scriptsize{Rank 1} & \scriptsize{Rank 3} & \scriptsize{Rank 1} & \scriptsize{Rank 3} \\
    \midrule
    Uy~\cite{uy-deformawareretrieval-eccv20}+NC~\cite{Yifan:NeuralCage:2020} & 0.480 & 0.582 & 0.575 & 0.662 & 0.589 & 0.717\\
    Ours Joint + NC \cite{Yifan:NeuralCage:2020} & \textbf{0.476} & 0.582 & \textbf{0.411} & \textbf{0.480} & \textbf{0.538} & \textbf{0.623}\\    
    \midrule
    Uy~\cite{uy-deformawareretrieval-eccv20}+DO & 0.584 & 0.707 & 0.452 & 0.533 & 0.633 & 0.763\\
    \textbf{Ours} + DO & \textbf{0.504} & \textbf{0.620} & \textbf{0.414} & \textbf{0.513} & \textbf{0.494} & \textbf{0.580}\\
    \textbf{Ours w/ L2} + DO & \textbf{0.484} & \textbf{0.586} &  &  & \textbf{0.485} & \textbf{0.560}\\
    \midrule
    Uy~\cite{uy-deformawareretrieval-eccv20}+DF & 0.965 & 1.067 & 1.561 & 1.678 & 0.829 & 0.913\\
    \textbf{Ours} & \textbf{0.763} & \textbf{0.906} & \textbf{0.696} & \textbf{0.848} & 0.\textbf{715} & \textbf{0.791}\\
    \textbf{Ours w/ L2} & \textbf{0.691} & \textbf{0.810} &  &  & \textbf{0.696} & \textbf{0.749}\\
    \midrule
    Uy~\cite{uy-deformawareretrieval-eccv20}+DF (No Conn.) & 1.107 & 1.252 & 1.728 & 1.830 & 1.480 & 1.656\\
    Rnd. Samp. (No Conn.) & 1.129 & 1.285 & 1.655 & 1.708 & 1.358 & 1.344\\
    \textbf{Ours} (No Conn.) & \textbf{0.757} & \textbf{0.920} & \textbf{0.708} & \textbf{0.847} & \textbf{0.846} & \textbf{0.981}\\
    \midrule    
    Uy~\cite{uy-deformawareretrieval-eccv20}+DF (Rnd. Seg.) &  &  &  &  &  & \\
    Rnd. Samp. (Rnd. Seg.) & 1.097 & 1.163 &  &  &  & \\
    \textbf{Ours} (Rnd. Seg.) & 0.775 & 0.802 &  &  &  & \\
    \bottomrule 
\end{tabularx}
\caption{Joint Training on different parameterizations. }
\label{tbl:diff_params}
}
\vspace{-\baselineskip} 
\end{table}
